A Modular-based Strategy for Mitigating Gradient Conflicts in Simultaneous Speech Translation

Simultaneous Speech Translation (SimulST) involves generating target language text while continuously processing streaming speech input, presenting significant real-time challenges. Multi-task learning is often employed to enhance SimulST performance but introduces optimization conflicts between primary and auxiliary tasks, potentially compromising overall efficiency. The existing model-level conflict resolution methods are not well-suited for this task which exacerbates inefficiencies and leads to high GPU memory consumption. To address these challenges, we propose a Modular Gradient Conflict Mitigation (MGCM) strategy that detects conflicts at a finer-grained modular level and resolves them utilizing gradient projection. Experimental results demonstrate that MGCM significantly improves SimulST performance, particularly under medium and high latency conditions, achieving a 0.68 BLEU score gain in offline tasks. Additionally, MGCM reduces GPU memory consumption by over 95\% compared to other conflict mitigation methods, establishing it as a robust solution for SimulST tasks.

==> None/fig2_pdf.tex <==
\begin{figure}[t]
\centering
\centering
\includegraphics[width=0.7\columnwidth]{figs/modular.pdf}
\caption{Gradient modularization. In a Transformer-based model, key components such as the attention mechanism can be divided into separate gradient modules for $Q$, $K$, $V$, and the output linear layer. Similar modularization is applied to the Feed Forward Network and Layer Normalization layers.}
\label{fig:modular}
\end{figure}

==> None/figduibi.tex <==
% 颜色定义
\definecolor{qgreen}{RGB}{226,240,217}
\definecolor{qyellow}{RGB}{255,242,204}
\definecolor{qorange}{RGB}{248,203,173}
\definecolor{qblue}{RGB}{189,215,238}
\definecolor{qmidgreen}{RGB}{169,209,142}
\definecolor{qmidyellow}{RGB}{255,217,102}
\definecolor{qpenorange}{RGB}{238,140,69}
\definecolor{qpenblue}{RGB}{68,114,196}
\definecolor{qkgreen}{RGB}{118,176,79}
\definecolor{qkorange}{RGB}{255,192,0}

\begin{figure}

\begin{tikzpicture}
% 控件定义
\tikzstyle{texttitle} = [font=\scriptsize,align=center]
\tikzstyle{textonly} = [font=\scriptsize,align=left]
\tikzstyle{sublayer} = [rectangle,draw,minimum width=2.4cm,rounded corners=5pt,align=center,inner sep=3pt,minimum height=0.8cm,font=\scriptsize];
\tikzstyle{subsublayer} = [rectangle,draw,minimum width=1.8cm,rounded corners=5pt,align=center,inner sep=3pt,minimum height=0.9cm,font=\scriptsize];
\tikzstyle{mycircle} = [circle,draw,minimum width=0.4cm,rounded corners=3pt,align=center,inner sep=3pt,minimum height=0.3cm,font=\small];
\tikzstyle{background} = [rectangle,draw,rounded corners=5pt,minimum width=2.4cm,minimum height=2.1cm,font=\footnotesize,align=center];
\tikzstyle{background_legend} = [rectangle,draw,rounded corners=3pt,minimum width=6cm,minimum height=0.5cm,font=\footnotesize,align=center];
\tikzstyle{back} = [rectangle,rounded corners=5pt,minimum width=3.2cm,minimum height=0.8cm,font=\footnotesize,align=center];
\tikzstyle{back1} = [rectangle,rounded corners=5pt,minimum width=8cm,minimum height=1.25cm,font=\footnotesize,align=center];
\tikzstyle{back2} = [rectangle,rounded corners=5pt,minimum width=8cm,minimum height=2.3cm,font=\footnotesize,align=center];
% 图形居中
\node[textonly] at (-4.2,0) {};
% Global Gradients
\node[back1,fill=gray!10](GG) at (0, 0){};
\node[sublayer,color=qgreen,fill=qgreen,fill opacity=1](SimulST) at ([xshift=-1.6cm, yshift=0.6cm]GG.south) {};
\node[texttitle, color=black] at ([yshift=-0.28cm]SimulST.north) {SimulST};
\node[texttitle] at ([yshift=0.24cm]SimulST.south) {
    \textcolor{black}{(}
    \textcolor{qpenorange}{0.5}
    \textcolor{black}{,}
    \textcolor{qpenorange}{0.4}
    \textcolor{black}{,}
    \textcolor{qpenblue}{0.7}
    \textcolor{black}{,}
    \textcolor{qpenblue}{0.4}
    \textcolor{black}{)}
  };
\node[sublayer,color=qyellow,fill=qyellow,fill opacity=1](SimulASR) at ([xshift=2.7cm, yshift=0.6cm]GG.south) {};
\node[texttitle, color=black] at ([yshift=-0.28cm]SimulASR.north) {SimulASR};
\node[texttitle] at ([yshift=0.24cm]SimulASR.south) {
    \textcolor{black}{(}
    \textcolor{qpenorange}{0.9}
    \textcolor{black}{,}
    \textcolor{qpenorange}{0.8}
    \textcolor{black}{,}
    \textcolor{qpenblue}{-0.9}
    \textcolor{black}{,}
    \textcolor{qpenblue}{0.7}
    \textcolor{black}{)}
  };
\node[mycircle,color=black,fill=white,thick](J1) at ([xshift=0.55cm,yshift=0.85cm]GG.south){};
\node[font=\scriptsize] at ([yshift=-0.2cm]J1.north) {\usym{1F5F8}};
\draw[stealth-stealth,color=black,line width=0.5pt] ([xshift=-0.35cm, yshift=-0.08cm] J1.south) -- ([xshift=0.35cm, yshift=-0.08cm] J1.south);
\node[texttitle, color=black] at ([yshift=-0.28cm]J1.south) {\textbf{0.42}};
\node[texttitle, color=black] at ([yshift=0.5cm]SimulST.north) {Primary Task};
\node[texttitle, color=black] at ([yshift=0.48cm]J1.north) {Cos Similarity};
\node[texttitle, color=black] at ([yshift=0.5cm]SimulASR.north) {Auxiliary Task};
\node[texttitle, color=black] at ([xshift=-0.6cm]SimulST.west) {Global\\Gradients};
% Local Gradients
\node[back2,fill=gray!10    ](LG) at ([yshift=-1.3cm]GG.south){};
\node[background,densely dashed,color=qkgreen,line width=0.5pt](ST) at ([xshift=-1.6cm, yshift=-1.15cm]LG.north) {};
\node[subsublayer,color=qorange,fill=qorange,fill opacity=1](ST_Encoder) at ([yshift=-0.5cm]ST.north) {};
\node[texttitle, color=black] at ([yshift=-0.35cm]ST_Encoder.north) {Encoder};
\node[texttitle] at ([yshift=0.3cm]ST_Encoder.south) {
    \textcolor{black}{(}
    \textcolor{qpenorange}{0.5 }
    \textcolor{black}{,}
    \textcolor{qpenorange}{ 0.4}
    \textcolor{black}{)}
  };
\node[subsublayer,color=qblue,fill=qblue,fill opacity=1](ST_Decoder) at ([yshift=0.5cm]ST.south) {};
\node[texttitle, color=black] at ([yshift=-0.35cm]ST_Decoder.north) {Decoder};
\node[texttitle] at ([yshift=0.3cm]ST_Decoder.south) {
    \textcolor{black}{(}
    \textcolor{qpenblue}{0.7 }
    \textcolor{black}{,}
    \textcolor{qpenblue}{ 0.4}
    \textcolor{black}{)}
  };
\node[background,densely dashed,color=qkorange,line width=0.5pt](ASR) at ([xshift=2.7cm, yshift=-1.15cm]LG.north) {};
\node[subsublayer,color=qorange,fill=qorange,fill opacity=1](ASR_Encoder) at ([yshift=-0.5cm]ASR.north) {};
\node[texttitle, color=black] at ([yshift=-0.35cm]ASR_Encoder.north) {Encoder};
\node[texttitle] at ([yshift=0.3cm]ASR_Encoder.south) {
    \textcolor{black}{(}
    \textcolor{qpenorange}{0.9 }
    \textcolor{black}{,}
    \textcolor{qpenorange}{ 0.8}
    \textcolor{black}{)}
  };
\node[subsublayer,color=qblue,fill=qblue,fill opacity=1](ASR_Decoder) at ([yshift=0.5cm]ASR.south) {};
\node[texttitle, color=black] at ([yshift=-0.35cm]ASR_Decoder.north) {Decoder};
\node[texttitle] at ([yshift=0.3cm]ASR_Decoder.south) {
    \textcolor{black}{(}
    \textcolor{qpenblue}{-0.9 }
    \textcolor{black}{,}
    \textcolor{qpenblue}{ 0.7}
    \textcolor{black}{)}
  };
\node[mycircle,color=black,fill=white,thick](J2) at ([xshift=0.55cm,yshift=-0.42cm]LG.north){};
\node[font=\scriptsize] at ([yshift=-0.2cm]J2.north) {\usym{1F5F8}};
\draw[stealth-stealth,color=black,line width=0.5pt] ([xshift=-0.35cm, yshift=-0.08cm] J2.south) -- ([xshift=0.35cm, yshift=-0.08cm] J2.south);
\node[texttitle, color=black] at ([yshift=-0.28cm]J2.south) {\textbf{0.77}};
\node[mycircle,color=red,fill=white,thick](J3) at ([xshift=0.55cm,yshift=0.8cm]LG.south){};
\node[font=\scriptsize,color=red] at ([yshift=-0.2cm]J3.north) {\usym{1F5F4}};
\draw[stealth-stealth,color=red,line width=0.5pt] ([xshift=-0.35cm, yshift=-0.08cm] J3.south) -- ([xshift=0.35cm, yshift=-0.08cm] J3.south);
\node[texttitle, color=red] at ([yshift=-0.28cm]J3.south) {\textbf{-0.35}};
% \draw ([xshift=-0.05cm,yshift=-0.05cm]J3.west) circle (2pt);
% \draw ([xshift=-0.5cm,yshift=-0.35cm]J3.west) circle (2pt);
% \draw ([xshift=-0.6cm,yshift=-0.6cm]J3.west) circle (2pt);
% \draw ([xshift=-0.4cm,yshift=-0.9cm]J3.west) circle (2pt);
\draw [-stealth,color=red,line width=0.9pt] ([xshift=-0.05cm,yshift=-0.05cm]J3.west) .. controls ([xshift=-0.5cm,yshift=-0.35cm]J3.west) and ([xshift=-0.6cm,yshift=-0.6cm]J3.west) .. ([xshift=-0.4cm,yshift=-0.9cm]J3.west);
\node[texttitle, color=red] at ([yshift=-0.9cm]J3.south) {Gradient Conflict};
\node[texttitle, color=black] at ([xshift=-0.6cm]ST.west) {Local\\Gradients};
% 单向箭头
\draw[->,color=qmidgreen,line width=2pt] ([yshift=-0.1cm] SimulST.south) -- ([yshift=0.1cm] ST_Encoder.north);
\draw[->,color=qmidyellow,line width=2pt] ([yshift=-0.1cm] SimulASR.south) -- ([yshift=0.1cm] ASR_Encoder.north);
\draw[-stealth,color=black,line width=0.7pt] (ST_Encoder.south) -- (ST_Decoder.north);
\draw[-stealth,color=black,line width=0.7pt] (ASR_Encoder.south) -- (ASR_Decoder.north);
% 图例
% \node[background_legend,densely dotted,color=black,line width=1pt](legend) at ([xshift=-1.7cm, yshift=1cm]SimulASR.north) {};
% \node[font=\scriptsize] at ([xshift=-2.7cm,yshift=-0.25cm]legend.north) {\usym{1F5F8}};
% \node[font=\scriptsize,color=red] at ([xshift=0.35cm,yshift=-0.25cm]legend.north) {\usym{1F5F4}};
% \node[anchor=west, text width=2.3cm,font=\scriptsize] at ([xshift=-2.5cm,yshift=-0.25cm]legend.north) {No Gradient Conflict};
% \node[anchor=west, text width=2.3cm,font=\scriptsize] at ([xshift=0.55cm,yshift=-0.25cm]legend.north) {Gradient Conflict};

\end{tikzpicture}
\caption{Comparison of global and local gradient conflicts using cosine similarity. The global gradients show no conflict (top). However, local gradients reveal conflicts between the decoders (bottom), illustrating the concept of gradient conflict masking.}
\label{fig1}
\end{figure}

==> None/figmodular.tex <==
\definecolor{qdorange}{RGB}{237,130, 57}
\definecolor{qdblue}{RGB}{ 91,155,213}
\definecolor{qdgreen}{RGB}{118,176, 80}
\definecolor{qorange}{RGB}{244,177,131}
\definecolor{qblue}{RGB}{143,170,220}
\definecolor{qgreen}{RGB}{169,209,142}
\definecolor{qsorange}{RGB}{251,229,214}
\definecolor{qsblue}{RGB}{222,235,247}
\definecolor{qsgreen}{RGB}{226,240,217}


\begin{figure}

\begin{tikzpicture}
\tikzstyle{textonly} = [font=\scriptsize,align=left]
\tikzstyle{sublayer} = [rectangle,draw,rounded corners=5pt,minimum width=4.62cm,minimum height=3.65cm,font=\footnotesize,align=center];
\tikzstyle{background1} = [rectangle,draw,rounded corners=5pt,minimum width=4.2cm,minimum height=1.22cm,font=\footnotesize,align=center];
\tikzstyle{background2} = [rectangle,draw,rounded corners=5pt,minimum width=4.2cm,minimum height=0.7cm,font=\footnotesize,align=center];
\tikzstyle{background3} = [rectangle,draw,rounded corners=5pt,minimum width=4.2cm,minimum height=0.7cm,font=\footnotesize,align=center];
\tikzstyle{middlesqurd} = [rectangle,draw,minimum width=0.3cm,rounded corners=2pt,align=center,inner sep=3pt,minimum height=0.3cm,font=\scriptsize];
\tikzstyle{module} = [rectangle,draw,minimum width=1.4cm,rounded corners=2pt,align=center,inner sep=3pt,minimum height=0.4cm,font=\scriptsize];
\tikzstyle{background_legend} = [rectangle,draw,rounded corners=3pt,minimum width=2.6cm,minimum height=2.6cm,font=\footnotesize,align=center];

\node[textonly] at (-4.2,0) {};
%
% \node[sublayer,color=black!25,line width=0.5pt](M3) at (-0.2,0.4) {};
% \node[sublayer,color=black!60,fill=white,line width=0.5pt](M2) at (0,0.2) {};
\node[sublayer,color=black,fill=white,line width=0.5pt](M1) at (0.2,0) {};
% Attention Mechanism
\node[background1,densely dashed,color=qdorange,line width=0.5pt](AM) at ([yshift=0.82cm]M1.south) {};
\node[textonly,fill=white,fill opacity=1] at ([xshift=0cm, yshift=0cm]AM.north) {Attention Mechanism};
\node[module,color=qsorange,fill=qsorange] at ([xshift=-1cm,yshift=-0.4cm]AM.north) {};
\node[middlesqurd,color=qorange,fill=qorange](Grad_Q) at ([xshift=-1cm,yshift=-0.4cm]AM.north) {};
\node[textonly] at ([xshift=-0.7cm]Grad_Q.west) {Q};
\node[module,color=qsorange,fill=qsorange] at ([xshift=-1cm,yshift=-0.92cm]AM.north) {};
\node[middlesqurd,color=qorange,fill=qorange](Grad_V) at ([xshift=-1cm,yshift=-0.92cm]AM.north) {};
\node[textonly] at ([xshift=-0.7cm]Grad_V.west) {V};
\node[module,color=qsorange,fill=qsorange] at ([xshift=1.3cm,yshift=-0.4cm]AM.north) {};
\node[middlesqurd,color=qorange,fill=qorange](Grad_K) at ([xshift=1.3cm,yshift=-0.4cm]AM.north) {};
\node[textonly] at ([xshift=-0.7cm]Grad_K.west) {K};
\node[module,color=qsorange,fill=qsorange] at ([xshift=1.3cm,yshift=-0.92cm]AM.north) {};
\node[middlesqurd,color=qorange,fill=qorange](Grad_L) at ([xshift=1.3cm,yshift=-0.92cm]AM.north) {};
\node[textonly] at ([xshift=-0.7cm]Grad_L.west) {O};
\node[middlesqurd,color=qorange,fill=qorange] at ([xshift=-0.3cm]Grad_Q.west) {};
\node[middlesqurd,color=qorange,fill=qorange] at ([xshift=0.3cm]Grad_Q.east) {};
\node[middlesqurd,color=qorange,fill=qorange] at ([xshift=-0.3cm]Grad_K.west) {};
\node[middlesqurd,color=qorange,fill=qorange] at ([xshift=0.3cm]Grad_K.east) {};
\node[middlesqurd,color=qorange,fill=qorange] at ([xshift=-0.3cm]Grad_V.west) {};
\node[middlesqurd,color=qorange,fill=qorange] at ([xshift=0.3cm]Grad_V.east) {};
\node[middlesqurd,color=qorange,fill=qorange] at ([xshift=-0.3cm]Grad_L.west) {};
\node[middlesqurd,color=qorange,fill=qorange] at ([xshift=0.3cm]Grad_L.east) {};
% FFN
\node[background3,densely dashed,color=qgreen,line width=0.5pt](F) at([yshift=0.6cm]AM.north) {};
\node[textonly,fill=white,fill opacity=1] at ([xshift=0cm, yshift=0cm]F.north) {Feed Forward Network};
\node[module,color=qsgreen,fill=qsgreen] at ([xshift=-0.8cm,yshift=-0.4cm]F.north) {};
\node[middlesqurd,color=qgreen,fill=qgreen](Grad_F) at ([xshift=-0.8cm,yshift=-0.4cm]F.north) {};
\node[textonly] at ([xshift=-0.85cm]Grad_F.west) {$W_1$};
\node[module,color=qsgreen,fill=qsgreen] at ([xshift=1.3cm,yshift=-0.4cm]F.north) {};
\node[middlesqurd,color=qgreen,fill=qgreen](Grad_A) at ([xshift=1.3cm,yshift=-0.4cm]F.north) {};
\node[textonly] at ([xshift=-0.85cm]Grad_A.west) {$W_2$};
\node[middlesqurd,color=qgreen,fill=qgreen] at ([xshift=-0.3cm]Grad_F.west) {};
\node[middlesqurd,color=qgreen,fill=qgreen] at ([xshift=0.3cm]Grad_F.east) {};
\node[middlesqurd,color=qgreen,fill=qgreen] at ([xshift=-0.3cm]Grad_A.west) {};
\node[middlesqurd,color=qgreen,fill=qgreen] at ([xshift=0.3cm]Grad_A.east) {};
% Layer Norm
\node[background2,densely dashed,color=qblue,line width=0.5pt](LN) at([yshift=0.6cm]F.north) {};
\node[textonly,fill=white,fill opacity=1] at ([xshift=0cm, yshift=0cm]LN.north) {Layer Norm};
\node[module,color=qsblue,fill=qsblue] at ([yshift=-0.4cm]LN.north) {};
\node[middlesqurd,color=qblue,fill=qblue](Grad_LN) at ([yshift=-0.4cm]LN.north) {};
\node[textonly] at ([xshift=-0.8cm]Grad_LN.west) {LN};
\node[middlesqurd,color=qblue,fill=qblue] at ([xshift=-0.3cm]Grad_LN.west) {};
\node[middlesqurd,color=qblue,fill=qblue] at ([xshift=0.3cm]Grad_LN.east) {};
% legend
\node[module,color=lightgray,fill=lightgray] at ([yshift=0.5cm]M1.north) {};

\end{tikzpicture}

\caption{Gradient modularization. As key components within the Transformer model, the attention mechanism can be divided into separate gradients for $Q$, $K$, $V$, and the Linear layers. The operation is similar in the FFN and Layer Normalization layers.}
\label{fig:modular}
\end{figure}
